Multigoal-oriented optimal control problems with nonlinear PDE constraints

In this work, we consider an optimal control problem subject to a nonlinear PDE constraint and apply it to the regularized $p$-Laplace equation. To this end, a reduced unconstrained optimization problem in terms of the control variable is formulated. Based on the reduced approach, we then derive an a posteriori error representation and mesh adaptivity for multiple quantities of interest. All quantities are combined to one, and then the dual-weighted residual (DWR) method is applied to this combined functional. Furthermore, the estimator allows for balancing the discretization error and the nonlinear iteration error. These developments allow us to formulate an adaptive solution strategy, which is finally substantiated via several numerical examples.

==> Proof.tex <==
The proof follows the same idea as in \cite{RanVi2013,EnLaWi18} but is presented for the completeness of presentation.
Define $e$ and $e^*$ as above.
Let $\overline{x}$, $x$, $\tilde{x}_h$  be defined as $\overline{x}:=(\overline{q},\overline{p})$, ${x}:=({q},{p})$, $\tilde{x}_h:=(\tilde{q}_h,\tilde{p}_h)$ and $m(x):= i(q)+j'(q)(p)$. Furthermore let $e_x$ be defined $e_x:= \overline{x}-\tilde{x}_h$.
It holds that
\begin{align} \label{Equation: Trapez of m}
	\begin{split}
m(\overline{x})-m(\tilde{x}_h)=& \int\limits_0^1m'(\tilde{x}_h+ s e_x)(e_x) \text{ d}s \\
=& \frac{1}{2}  \big( m'(\tilde{x}_h)(e_x) d s + m'(\overline{x})(e_x)\big) +\frac{1}{2}\int\limits_0^1m'''(\tilde x_h+se_x)(e_x,e_x,e_x)s(s-1)\text{ d}s.
\end{split}
\end{align}

%By carefully inspecting $\frac{1}{2}\int\limits_0^1m'''(\tilde x_h+se_x)(e_x,e_x,e_x)s(s-1)\text{ d}s$ it follows that
% it coincides with $\mathcal{R}^{(3)}$.
 By carefully inspecting $m'''(\tilde x_h+se_x)(e_x,e_x,e_x)$ it follows that
 $$m'''(\tilde x_h+se_x)(e_x,e_x,e_x)=(m'''_{qqq}+3m'''_{qqp}+3m'''_{qpp}+m'''_{ppp})(\tilde x_h+se_x)(e_x,e_x,e_x),$$
 and since $m''_{pp}=0$ and $m'_p(\tilde x_h+se_x)(e_x)=j'(\tilde{q}_h +s(e))(e^*)$ , we obtain 
  $$m'''(\tilde x_h+se_x)(e_x,e_x,e_x)=i'''(\tilde{q}_h+se)(e,e,e)
  +j''''(\tilde{q}_h+se)(e,e,e,\tilde{p}_h+se^*)+3j'''(\tilde{q}_h +s(e))(e,e,e^*),$$ and therefore $\frac{1}{2}\int\limits_0^1m'''(\tilde x_h+se_x)(e_x,e_x,e_x)s(s-1)\text{ d}s$ coincides with \eqref{Error Estimator: Remainderterm}.
  For the part $m'(\overline{x})(e_x)$ of \eqref{Equation: Trapez of m} we can deduce that
$$m'(\overline{x})(e_x)=\underbrace{i'(\overline{q})+j''(\overline{q})(e,\overline{p})}_{=0}+\underbrace{j'(\overline{q})(e^*)}_{=0}=0.$$
Finally \eqref{Equation: Trapez of m} reduces to  the following identity
$$m(\overline{x})-m(\tilde{x}_h) = \frac{1}{2}  m'(\tilde{x}_h)(e_x) + \mathcal{R}^{(3)}.$$
and therefore we get
\begin{align*}
i(\overline{q})-i(\tilde{q}_h)=m(\overline{x})-\underbrace{j'(\overline{q})(\overline{q})}_{=0}-m(\tilde{x}_h)+\underbrace{j'(\tilde{q}_h)(\tilde{p}_h)}_{\rho (\tilde{q}_h)(\tilde{p}_h)}.
\end{align*}
This proofs the theorem after verifying that $m'(\tilde{x}_h)(e_x)= \rho(\tilde{q}_h)(\overline{p}-\tilde{p}_h)+\rho^*(\tilde{q}_h,\tilde{p}_h)(\overline{q}-\tilde{q}_h) $.


